VeriChat: An Agentic Conversational AI Assistant for Hardware Security Verification

Hardware security verification is a multi-stage process in which engineers must navigate complex design analyses, threat considerations, and verification strategies. They often need security-focused guidance, yet current verification environments provide little structured support for such assistance. Although conversational AI could offer such on-demand assistance, directly using general-purpose chatbots like ChatGPT or Gemini is risky due to their tendency to hallucinate and their reliance on static, outdated knowledge. We present VeriChat, a domain-specialized conversational assistant designed to support, rather than replace, existing verification workflows by providing context-aware security guidance. VeriChat employs a retrieval-augmented, multi-agent workflow in which three specialized agents collaboratively minimize hallucinations while improving the transparency and reliability of the response. Beyond question answering, VeriChat integrates open-source EDA tools, including Icarus Verilog, Yosys, and SymbiYosys, to perform syntax checking, synthesis analysis, simulation, and formal verification directly on user-provided RTL designs. Evaluated using a comprehensive methodology, VeriChat achieves a Faithfulness score of 87.73%, significantly outperforming the leading proprietary models. We demonstrate the framework through a hardware Trojan detection case study on an AES S-Box IP, where VeriChat autonomously identifies, simulates, and formally proves a covert key-leakage vulnerability through a multi-turn conversational workflow.

==> algorithm_bugbench.tex <==

\begin{algorithm}
\caption{LLM-Driven RTL Bug Validation Framework with Prompt-Level Modeling}
\begin{algorithmic}[1]
\Require RTL Design $\mathcal{R}$, Bug Explanation $\mathcal{B}$, LLM, Static Syntax Checker \texttt{SYN}, EDA Simulator \texttt{SIM}
\Ensure Validation Result $\mathcal{V} \in \{\texttt{MATCH}, \texttt{MISMATCH}, \texttt{ROI\_IMPERFECT}\}$

\State $k \gets 0$; \quad $\text{MAX\_ITER} \gets N$
\While{$k < \text{MAX\_ITER}$}
    \Comment{\textbf{Flow 1: Scenario Generation and Simulation}}
    \State $\mathcal{P}_1 \gets \texttt{BuildScenarioPrompt}(\mathcal{R}, \mathcal{B})$
    \State $\mathcal{S}_{\text{test}} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_1)$

    \While{$\neg \texttt{CriticApprove}(\mathcal{S}_{\text{test}})$}
        \State $\mathcal{F}_{\text{scenario}} \gets \texttt{ScenarioFeedback}(\mathcal{S}_{\text{test}})$
        \State $\mathcal{P}_1 \gets \texttt{UpdatePrompt}(\mathcal{P}_1, \mathcal{F}_{\text{scenario}})$
        \State $\mathcal{S}_{\text{test}} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_1)$
    \EndWhile

    \State $\mathcal{P}_2 \gets \texttt{BuildTestbenchPrompt}(\mathcal{R}, \mathcal{B}, \mathcal{S}_{\text{test}})$
    \State $\mathcal{T}_{\text{raw}} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_2)$

    \While{$\neg \texttt{IsSyntaxValid}(\texttt{SYN}, \mathcal{T}_{\text{raw}})$}
        \State $\mathcal{F}_{\text{syntax}} \gets \texttt{ParseSyntaxError}(\texttt{SYN}, \mathcal{T}_{\text{raw}})$
        \State $\mathcal{P}_2 \gets \texttt{UpdatePrompt}(\mathcal{P}_2, \mathcal{F}_{\text{syntax}})$
        \State $\mathcal{T}_{\text{raw}} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_2)$
    \EndWhile

    \State $(\mathcal{M}_{\text{sim}}, \mathcal{M}_{\text{blank}}, \texttt{status}) \gets \texttt{RunSimulation}(\texttt{SIM}, \mathcal{T}_{\text{raw}}, \mathcal{R})$
    \If{$\texttt{status} == \texttt{TIMEOUT}$}
        \State $k \gets k + 1$
        \State \textbf{continue}
    \EndIf

    \Comment{\textbf{Flow 2: Golden Monitor Generation and Validation}}
    \State $\mathcal{P}_3 \gets \texttt{BuildGoldenMonitorPrompt}(\mathcal{R}, \mathcal{B}, \mathcal{S}_{\text{test}}, \mathcal{M}_{\text{blank}})$
    \State $\mathcal{M}_{\text{golden}} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_3)$

    \State $\mathcal{P}_4 \gets \texttt{BuildROIPrompt}(\mathcal{M}_{\text{golden}}, \mathcal{B})$
    \State $\mathcal{R}_{\text{ROI}} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_4)$

    \State $\mathcal{P}_5 \gets \texttt{BuildValidationPrompt}(\mathcal{M}_{\text{sim}}, \mathcal{R}_{\text{ROI}}, \mathcal{B})$
    \State $\mathcal{V} \gets \texttt{LLM\_Infer}(\text{LLM}, \mathcal{P}_5)$

    \If{$\mathcal{V} == \texttt{MATCH}$}
        \State \Return $\texttt{MATCH}$
    \ElsIf{$\mathcal{V} == \texttt{MISMATCH}$}
        \State $k \gets k + 1$
        \State \textbf{continue}
    \ElsIf{$\mathcal{V} == \texttt{ROI\_IMPERFECT}$}
        \State $\mathcal{F}_{\text{roi}} \gets \texttt{ROI\_Feedback}(\mathcal{M}_{\text{golden}}, \mathcal{R}_{\text{ROI}})$
        \State $\mathcal{P}_3 \gets \texttt{UpdatePrompt}(\mathcal{P}_3, \mathcal{F}_{\text{roi}})$
        \State \textbf{continue}
    \EndIf
\EndWhile

\State \Return \texttt{FAILED}
\end{algorithmic}
\end{algorithm}
